Stochastic Thermodynamics of Non-reciprocally Interacting Particles and Fields

Nonreciprocal interactions that violate Newton's law 'actio=reactio' are ubiquitous in nature and are currently intensively investigated in active matter, chemical reaction networks, population dynamics, and many other fields. An outstanding challenge is the thermodynamically consistent formulation of the underlying stochastic dynamics that obeys local detailed balance and allows for a rigorous analysis of the stochastic thermodynamics of non-reciprocally interacting particles. Here, we present such a framework for a broad class of active systems and derive by systematic coarse-graining exact expressions for the macroscopic entropy production. Four independent contributions to the thermodynamic dissipation can be identified, among which the energy flux sustaining vorticity currents manifests the presence of non-reciprocal interactions. Then, Onsager's non-reciprocal relations, the fluctuation-response relation, the fluctuation relation and the thermodynamic uncertainty relations for non-reciprocal systems are derived. Finally, we demonstrate that our general framework is applicable to a plethora of active matter systems and chemical reaction networks and opens new paths to understand the stochastic thermodynamics of non-reciprocally interacting many-body systems.

==> abbrev.tex <==

% Atul's commands

\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}
\renewcommand\thesubsubsection{\textbf{\Alph{subsubsection}}}

\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}


\newcommand{\amnote}[1]{\note{#1}}

\newcommand{\dr}{d\mathbf{r}^2\:}
\newcommand{\dt}{\partial_t}
\newcommand{\funcder}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\partder}[2]{\frac{\partial #1}{\partial #2}}

\newcommand{\crt}{\hat{\eta}^\dag_{i}} 
\newcommand{\anh}{\hat{\eta}_{i}}
\newcommand{\numbop}{\hat{N}_{\theta_\alpha}} 
\newcommand{\noiseop}{\hat{\chi}^{i, j}_{\theta_\alpha}}
\newcommand{\noiseopcontcont}{\hat{\chi}\left(\mathbf{r}, \theta\right)}
\newcommand{\noiseopcontdisct}{\hat{\chi}_{\theta_{\alpha}} \left(\mathbf{r}\right)}
\newcommand{\noiseopcontdisctlong}[1]{\hat{\chi}_{#1}\left(\mathbf{r} \right)}
\newcommand{\denseopcont}{\eta \left(\mathbf{r}, \theta\right)}
\newcommand{\numbopdot}{\dot{\hat{N}}_{i, j, \theta_\alpha}} 
\newcommand{\noiseopdot}{\dot{\hat{\chi}}^{i, j}_{\theta_\alpha}}
\newcommand{\dens}{N_{i}^\#}
\newcommand{\denscontcont}{{\eta}\left( \mathbf{r}, \theta \right)}
\newcommand{\denscontdisct}{{\eta_{\theta_\alpha}}\left( \mathbf{r} \right)}
\newcommand{\mucontdisct}{{\mu}_{\theta_\alpha}\left( \mathbf{r} \right)}
\newcommand{\mucontdisctlong}[1]{{\mu}_{#1}\left( \mathbf{r} \right)}
\newcommand{\mucontcont}{{\mu}\left( \mathbf{r}, \theta \right)}
\newcommand{\denscontdisctlong}[1]{{\eta_{#1}}\left( \mathbf{r} \right)}
\newcommand{\magcont}{\mathbf{m}\left(\mathbf{r} \right)}
\newcommand{\magcontx}{m^x\left(\mathbf{r} \right)}
\newcommand{\magconty}{m^y\left(\mathbf{r} \right)}
\newcommand{\magNcont}[1]{\mathbf{m}_{#1}\left(\mathbf{r} \right)}
\newcommand{\magNcontx}[1]{m_{#1}^x\left(\mathbf{r} \right)}
\newcommand{\magNconty}[1]{m_{#1}^y\left(\mathbf{r} \right)}
\newcommand{\orientdisct}{\hat{\mathbf{u}}_{\theta_\alpha}}
\newcommand{\orientcont}{\hat{\mathbf{u}}_{\theta}}
\newcommand{\orientcontx}{\hat{u}_{\theta}^x}
\newcommand{\orientconty}{\hat{u}_{\theta}^y}
\newcommand{\maglong}{\mathbf{m}^\parallel \left(\mathbf{r} \right)}
\newcommand{\magtrans}{\mathbf{m}^\perp \left( \mathbf{r} \right)}
\newcommand{\denscontcontlong}[1]{{\eta}\left( #1 \right)}
\newcommand{\rhocont}{{\rho(\mathbf{r})}}
\newcommand{\polcont}{{\mathbf{P}\left(\mathbf{r}\right)}}
\newcommand{\magcontmod}{{m}}
\newcommand{\polcontmod}{{P}}
\newcommand{\polcontparll}{{P^\parallel\left(\mathbf{r}\right)}}
\newcommand{\polcontperp}{{P^\perp \left(\mathbf{r}\right)}}
\newcommand{\polcontx}{{P^x\left(\mathbf{r}\right)}}
\newcommand{\polconty}{{P^y\left(\mathbf{r}\right)}}
\newcommand{\densdot}{\dot{{\eta}}_{i, j, \theta_\alpha}}
\newcommand{\state}{i, j, \theta_\alpha} 
\newcommand{\bra}{|\dens \rangle} 
\newcommand{\ket}{\langle \dens|} 
\newcommand{\bralong}[1]{|\dens_{#1} \rangle} 
\newcommand{\ketlong}[1]{\langle \dens_{#1}|} 
\newcommand{\braplus}{|\dens + 1\rangle} 
\newcommand{\ketplus}{\langle \dens + 1|} 
\newcommand{\braminus}{|\dens - 1 \rangle} 
\newcommand{\ketminus}{\langle \dens - 1|} 

\newcommand{\crtlong}[2]{{(\hat{\eta}_{#1}^{#2})}^\dag} 
\newcommand{\anhlong}[2]{\hat{\eta}_{#1}^{#2}}
\newcommand{\numboplong}[2]{\hat{N}_{#1}^{#2}} 
\newcommand{\noiseoplong}[2]{\hat{\chi}^{#1}_{#2}}
\newcommand{\statelong}[1]{#1} 
\newcommand{\denslong}[2]{N_{#1}^{#2}} 
\newcommand{\densoplong}[1]{\hat{N}_{#1}} 
\newcommand{\densoplongg}[2]{{{\hat{N}}_{#1}}^{#2}} 


\newcommand{\energychangehop}{\Delta E\left(\{i + a, j + b, \theta_\alpha\} \leftarrow \{i, j, \theta_\alpha\}\right)}
\newcommand{\energychangetumble}{\Delta E \left(\{i, j, \theta_{\alpha \pm 1}\} \leftarrow \{i, j, \theta_\alpha\}\right)}

\newcommand{\energychangehoplong}[2]{\Delta E\left(\left \{#1\right \} \leftarrow \left \{#2 \right \}\right)}
\newcommand{\energychangetumblelong}[2]{\Delta E \left(\left \{#1 \right \} \leftarrow \left \{#2 \right \}\right)}

\newcommand{\interactionenergyparticle}{\sum_{\theta_{\omega}} V_{\theta_{\alpha}\theta_{\omega}}  \crtlong{i, j, \theta_{\omega}} \anhlong{i, j, \theta_{\omega}}}

\newcommand{\interactionenergyparticlelong}[3]{\sum_{\theta_{\omega}} V_{\theta_{#3} \theta_{\omega}}  \crtlong{#1,#2,\theta_{\omega}} \anhlong{#1, #2, \theta_{\omega}}}



